Coronal rain as a marker for coronal heating mechanisms

Reported observations in H-alpha, Ca II H and K or or other chromospheric lines of coronal rain trace back to the days of the Skylab mission. Offering a high contrast in intensity with respect to the background (either bright in emission if observed at the limb, or dark in absorption if observed on disk) these cool blobs are often observed falling down from high coronal heights above active regions. A physical explanation for this spectacular phenomenon has been put forward thanks to numerical simulations of loops with footpoint concentrated heating, a heating scenario in which cool condensations naturally form in the corona. This effect has been termed 'catastrophic cooling' and is the predominant explanation for coronal rain. In this work we further investigate the link between this phenomenon and the heating mechanisms acting in the corona. We start by analyzing observations of coronal rain at the limb in the Ca II H line performed by the SOT instrument on board of the Hinode satellite. We then compare the observations with 1.5-dimensional MHD simulations of loops being heated by small-scale discrete events concentrated towards the footpoints (that could come, for instance, from magnetic reconnection events), and by Alfven waves generated at the photosphere. It is found that if a loop is heated predominantly from Alfven waves coronal rain is inhibited due to the characteristic uniform heating they produce. Hence coronal rain may not only point to the spatial distribution of the heating in coronal loops but also to the agent of the heating itself. We thus propose coronal rain as a marker for coronal heating mechanisms.

==> table1.tex <==
\ProvidesFile{tab1.tex}%
 [2003/12/12 5.2/AAS markup document class]%

\begin{deluxetable}{ccccc}
\tabletypesize{\scriptsize}
%\rotate
\tablecaption{Falling velocities for coronal rain observed by Hinode/SOT}
\tablewidth{0pt}
\tablehead{
\colhead{Loop} & \colhead{Apex} & \colhead{Footpoint} & \colhead{Free fall ($v_{0}$=0)} 
}
\startdata
left & 50 - 70 & 115 & 115 \\
middle & 30 - 50 & 80 - 140 & 90 - 150 \\
 & -25 & \\
right & 60 - 70 & 15 $\rightarrow$ 105 & 45  \\
\enddata
\tablecomments{Estimated velocities of coronal rain for the 3 loops of Fig. \ref{f01}. ``Left", ``Middle" and ``right" denote, respectively, the loops in the left, middle and right panels of that figure. The velocities are calculated by estimating the slopes in the length - time diagrams. Speeds at the top part and bottom part of the loops are written in the ``apex" and ``footpoint" columns respectively. The ``free fall" column is the velocity calculated assuming free fall and no initial speed. Positive values denote downward motions. In the loop of the middle panel an upward motion at a velocity of $\sim$ 25 km s$^{-1}$ is observed on the top part of the loop. In the loop of the right panel a deceleration to a velocity of $\sim15$ km s$^{-1}$ is clearly observed halfway down the loop. It then accelerates again to $\sim105$ km s$^{-1}$. The free fall velocity for this case is calculated from the time of the start of this acceleration. \label{table1}}
\end{deluxetable}

%\end{document}

\endinput

